Unsupervised Contrastive Hashing for Cross-Modal Retrieval in Remote Sensing

The development of cross-modal retrieval systems that can search and retrieve semantically relevant data across different modalities based on a query in any modality has attracted great attention in remote sensing (RS). In this paper, we focus our attention on cross-modal text-image retrieval, where queries from one modality (e.g., text) can be matched to archive entries from another (e.g., image). Most of the existing cross-modal text-image retrieval systems in RS require a high number of labeled training samples and also do not allow fast and memory-efficient retrieval. These issues limit the applicability of the existing cross-modal retrieval systems for large-scale applications in RS. To address this problem, in this paper we introduce a novel unsupervised cross-modal contrastive hashing (DUCH) method for text-image retrieval in RS. To this end, the proposed DUCH is made up of two main modules: 1) feature extraction module, which extracts deep representations of two modalities; 2) hashing module that learns to generate cross-modal binary hash codes from the extracted representations. We introduce a novel multi-objective loss function including: i) contrastive objectives that enable similarity preservation in intra- and inter-modal similarities; ii) an adversarial objective that is enforced across two modalities for cross-modal representation consistency; and iii) binarization objectives for generating hash codes. Experimental results show that the proposed DUCH outperforms state-of-the-art methods. Our code is publicly available at https://git.tu-berlin.de/rsim/duch.

==> sections/1_intro_old.tex <==
\section{Introduction}
\label{sec:intro}
%@Mahdyar: I think there is a significant logic problem here: we talk on hashing, and then multimodal and then supervised hashing. I think that intro of journal paper is much better. as an example, where each bit represents a semantic feature or a combination of features is misleading. We can much better sentences for hashing motivation and desciption in the journal paper.
The increased number of recent Earth observation satellite missions has led to the significant growth of remote sensing (RS) image archives. Thus, the development of scalable and accurate retrieval systems (which aim at searching for semantically similar data with respect to a given query) for massive archives is one of the most important research topics in RS. 

Deep hashing methods are common approaches for scalable retrieval systems, where the semantic representation is learned as binary hash codes. The binary hash codes are generated for each sample, where each bit represents a semantic feature or a combination of features. Retrieval scalability and computation efficiency are achieved by hash tables lookup and calculation of hamming distances. Lai et al. \cite{lai2015simultaneous} introduced a deep learning-based method for learning hash codes based on triplet-loss. For a reference image (i.e., anchor) in each considered tuple of images, the triplet loss pulls a similar image (i.e., positive) closer to a reference while pushes a dissimilar image farther. Most of the existing hashing-based retrieval systems in RS are designed as uni-modal and consider only a single modality of data \cite{cao2020enhancing} (e.g., Sentinel-2 images). 

%connection from previous paragraph is not existing. In addition, why do we talk here voice-image retrieval? you sometime suse past tense, sometimes use presnet tense when you refer to soa- we need to fix it. it should be either present or past for all ...
Unlike RS, in the computer vision (CV) community, the use of multimodal data is more extended, and the importance of cross-modal representation learning is widely studied \cite{chen2020deep,cheng2021deep,xie2020multi}. In multimodal systems, one modality contains semantically similar counterparts in other modalities. Such multimodal data, when jointly considered, can allow rich characterization of each modality by leveraging the complementary information embedded in other modalities. Multimodal systems aim to allow accurate retrieval by jointly considering different data modalities (i.e., image and text), whereas cross-modal systems aim to search semantically similar samples in one modality by considering a query from another modality. Most existing methods in CV rely on label information to learn multimodal retrieval systems. In \cite{chen2020deep} a triplet-based method is introduced for voice-image retrieval. Cheng et al. \cite{cheng2021deep} used a semantic alignment mechanism based on attention and gate mechanisms for text-image retrieval. Xie et al. \cite{xie2020multi} proposed a multi-task consistency-preserving adversarial hashing (CPAH) that separates the feature representations into modality-specific and modality-common features, exploiting label information to learn consistent modality-specific representations. An adversarial learning strategy enforces inter-modality semantic consistency. 

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.85\linewidth]{images/main_diagram_2.pdf}
  \caption{
Block diagram of the proposed method. In the feature extraction module, the modality-specific encoders $net_{img}$ and $net_{txt}$ extract deep embedding for image and text modalities, respectively. The hashing module learns two hash functions $f$ and $g$ from the input embedding. Discriminator $D$ enforces the adversarial objective between two modalities for cross-modal representation consistency.}
  \label{fig:main-diagram}
\end{figure*}

%unclear for me the connection of previous paragraph to that one... 
The supervised hashing methods use label information, which is not always available for large RS archives, and collecting labels for such massive archives may not be feasible. Several unsupervised and self-supervised methods have been proposed in CV to overcome this limitation, where the only available information is the image and text alignment \cite{chen2020improved,chen2020simple,he2020momentum,jung2021contrastive,su2019deep}. Recently, contrastive-learning-based methods gain the popularity \cite{chen2020improved,chen2020simple,he2020momentum}. In \cite{chen2020simple}, an unsupervised contrastive learning is introduced, aiming to learn a metric space in which a sample is closer to its augmentations (i.e., different views) than all the other samples in the batch. The augmentations are obtained by applying flipping, rotation, and cropping. Jung et al. \cite{jung2021contrastive} proposed to use geographically close images as different views for a uni-modal self-supervised representation learning. Su et al. \cite{su2019deep} introduced a deep joint-semantics reconstructing hashing (DJSRH) method to learn binary codes that preserve the neighborhood structure in the original data. To this end, DJSRH learns a mapping from different modalities into a joint-semantics affinity matrix. Liu et al. \cite{liu2020joint} proposed a joint-modal distribution-based similarity weighting (JDSH) method based on DJSRH, exploiting an additional objective based on cross-modal semantic similarities among samples.


The existing unsupervised contrastive learning methods mainly rely on cross-modal (inter-modality) contrastive objectives to obtain consistent representations across different modalities, while the intra-modal contrastive objectives are ignored. In this paper, we propose a novel unsupervised cross-modal contrastive hashing (DUCH) method that takes to account inter- and intra-modality contrastive objectives for representation learning. %To this end, the proposed DUCH consists of two modules: 1) the feature extraction module consists of modality-specific encoders to generate the uni-modal deep representation; 2) the hashing module that aims at learning joint feature representations (in terms of binary hash codes) between image and text (i.e., captions) modalities by simultaneously preserving the semantic discrimination and modality-invariance in an end-to-end manner. 
In detail, we introduce a novel multi-objective loss function that consists of: 1) intra- and inter-modal contrastive objectives that enable similarity preservation within and between modalities; 2) an adversarial objective enforcing cross-modal representation consistency; 3) binarization objectives to generate representative binary hash codes. %We demonstrate the effectiveness of such additional objectives. %The rest of paper is organized as follows: Section \ref{sec:method} explains the architecture of proposed method, Section \ref{sec:experiments} describes experimental setup and data, Section \ref{sec:results} provides experimental results, and Section \ref{sec:conclusion} concludes the paper.
%\vspace{-0.5cm}

==> sections/excluded_table_arch.tex <==

\begin{table}[htbp]
    \renewcommand{\arraystretch}{1}
    \setlength{\tabcolsep}{5pt}
    \centering
    \small
    \caption{Network configuration of proposed DUCH. $B$ is the length of binary hash code[@G??].}
    \label{tab:architecture-modules}
    \begin{tabular}{l|c|c|c}
        \hline
        Module & Layer & Activation & Size \tabularnewline
        \hline\hline
        
        \multirow{3}{*}{Image Hashing Network}
        & $fc_1$ & $relu$ & $4096$ \\
        \cline{2-4}
        & $BatchNorm$ & - & - \\
        \cline{2-4}
        & $fc_2$ & $tanh$ & $B$ \\
        \hline\hline
        
        \multirow{3}{*}{Text Hashing Network}
        & $fc_1$ & $relu$ & $4096$ \\
        \cline{2-4}
        & $BatchNorm$ & - & - \\
        \cline{2-4}
        & $fc_2$ & $tanh$ & $B$ \\
        \hline\hline
        
        \multirow{3}{*}{Discriminator}
        & $fc_1$ & $ReLU$ & $B \times 2$ \\
        \cline{2-4}
        & $BatchNorm$ & - & - \\
        \cline{2-4}
        & $fc_2$ & - & $B$ \\
        \hline
    \end{tabular}
\end{table}


You: @G: why the embedding sizes are different from what you mentioned in the text?
Oct 7, 2021 1:24 AM • Edit • Delete
You: mage embedding size was $d_i=512$
Oct 7, 2021 1:25 AM • Edit • Delete
You: We obtained sentence embeddings in the size of $d_t=768$
Oct 7, 2021 1:25 AM • Edit • Delete

==> sections/intro_back.tex <==
\section{Introduction}
\label{sec:intro}

% Introduction
% introduce problems, motivate our work

%In recent years the volume of remote sensing (RS) image archives has significantly increased. In 2018 German Aerospace Center (DLR) predicted the German Satellite Data Archive to reach 180 petabyptes by 2030. \cite{dlr2018}. Accurate scalable content-based retrieval is essential for such huge archives.
 
%Content-based retrieval (CBR) aims to find most similar samples with respect to the query sample in large archives. All samples are encoded according to their semantic representations. Similarity between samples is defined by distance metric, such as Euclidean or Hamming distances. Most CBR systems in RS operate only with images. For instance, Cao et al. \cite{cao2020enhancing} use a triplet metric learning for CBR.

The increased number of recent Earth observation satellite missions has led to the significant growth of remote sensing (RS) image archives. Thus, the development of scalable and effective content-based retrieval (CBR) systems (which aims at searching for semantically similar data to a given query) in massive archives of images is one of the growing research interests in RS. Most existing CBR systems in RS are designed uni-modal and consider only a single modality \cite{cao2020enhancing} (e.g., Sentinel-2 images). Multimodal systems aim to allow accurate retrieval by jointly considering different data modalities (i.e., image and text), whereas cross-modal systems aim to search semantically similar samples in one modality by considering a query from another modality.

%Extracted hash representations of data samples are organized in hash tables.
Content-based hashing methods is one of CBR approaches for the semantic representation of information. Binary hash codes are generated for each sample, where each bit represent a semantic feature or a combination of features. Retrieval scalability and computation efficiency are achieved by hash tables lookup and calculation of hamming distances. Lai et al. \cite{lai2015simultaneous} were among the first to introduce a deep learning framework for hashing based on triplet-loss. Triplet-loss arranges similar samples close to each other in the feature space and far from dissimilar samples. It is achieved by selection of data triplets, containing anchor sample, positive (similar) sample and negative (dissimilar) sample.

%Supervised retrieval of multi-modal data is a well-studied topic in computer vision.
Data samples of one modality may have semantically similar counterparts in other modalities. These counterparts contain additional knowledge that can be used for improved representation learning. The most of state-of-the-art supervised multi-modal retrieval methods are based on the triplet-loss. As an example, in \cite{chen2020deep} a voice-image triplet-based retrieval is introduced. Cheng et al. \cite{cheng2021deep} improve text-image retrieval with aid of semantic alignment mechanism based on attention and gate mechanisms. Xie et al. \cite{xie2020multi} prposed a multi-task consistency-preserving adversarial hashing (CPAH) method. for feature consistency preservation, CPAH separates the feature representations into modality specific and modality common features. Furthermore, CPAH uses label information to train separate modality and feature classifiers, resulting in generating representative binary hash codes. 

Such supervised hashing methods use label information, which is not always available for large RS archives, and manual labeling of such massive archives is infeasible. To overcome such a limitation, several methods exploited unsupervised or self-supervised learning methods. No label information is used in the unsupervised methods, and the only available information is the image and text alignment. Recently, contrastive-learning-based methods such as SimCLR \cite{chen2020simple} and MoCo \cite{he2020momentum} \cite{chen2020improved} gain the popularity. In unsupervised contrastive learning, the model is trained to learn a metric space, where a sample is closer to its augmentations (i.e., different views) than all the other samples in the training set. In SimCLR and MoCo frameworks such augmentations are obtained by applying flipping, rotation and cropping to generate different image views. Jung et al. \cite{jung2021contrastive} use similarity of geographically close images for uni-modal self-supervised learning. A Multi-modal self-supervised learning approach is introduced in \cite{zhang2021cross}, where intra- and inter-modal contrastive losses are used for mutual information maximization in text-to-image generation task. Heidler et al. \cite{heidler2021self} propose a multi-modal framework for audio-visual embeddings generation. Su et al. \cite{su2019deep} introduced Deep Joint-Semantics Reconstructing Hashing (DJSRH) method. DJSRH is using cosine similarities matrices of batches to learn data samples affinity and improve unsupervised hash generation. Liu et al. \cite{liu2020joint} proposed a joint-modal distribution-based similarity weighting (JDSH) method to improve DJSRH. JDSH make use of an additional learning objective according to sample similarity magnitudes.



To address the aforementioned problems, we introduce a self-supervised deep cross-modal hashing system designed for retrieval in RS and CV. Our method achieves scalable cross-modal retrieval by utilizing multi-term contrastive loss for hashing. For hashing we use semantic embeddings generated by pretrained modality encoder networks. Next, semantic continuous binary-like features are generated via contrastive learning. Finally, generated continious features are quantized to obtain binary hash codes.

The rest of paper is organized as follows: Section \ref{sec:method} explains the architecture of proposed method, Section \ref{sec:experiments} describes experimental setup and data, Section \ref{sec:results} provides experimental results, and Section \ref{sec:conclusion} concludes the paper.

==> sections/tables.tex <==
\begin{table}
% see /data/out_table.csv
\setlength{\tabcolsep}{5pt}
\centering

\caption{The mAP@20 results for image-to-text ($I \to T$) and text-to-image ($T \to I$) retrieval tasks.}
\small
\label{tab:retrieval-performance}
\def\arraystretch{1.0}
\begin{tabular}{c|l|cccc} 
\hline
% header
Task & Method & $B$=16 & $B$=32 & $B$=64 & $B$=128  \\ 
\hline\hline
% I2T
\multirow{4}{*}{$I\to T$}        

& CPAH      & 0.428 & 0.587 &0.636 & 0.696 \\
& DJSRH       & 0.411 & 0.665 & 0.688 & 0.722  \\
& JDSH      & 0.385 & 0.720 & 0.796 & 0.815  \\
& DUCH         & \textbf{0.684} & \textbf{0.791} & \textbf{0.836} & \textbf{0.829}  \\
\hline\hline

% T2I
\multirow{4}{*}{$T\to I$}

& CPAH      & 0.452 & 0.598 & 0.667 & 0.706  \\
& DJSRH      & 0.422 & 0.685 & 0.705 & 0.733  \\
& JDSH      & 0.418 & 0.751 & 0.799 & 0.815 \\
& DUCH        & \textbf{0.697} & \textbf{0.780} & \textbf{0.824} & \textbf{0.826}  \\
\hline
\end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}
\centering
\small
\caption{The mAP@20 results for image-to-text ($I \to T$) and text-to-image ($T \to I$) retrieval tasks under different configurations of the proposed DUCH when $B=64$.}
\label{tab:ablation-study}
\def\arraystretch{1.05}
\begin{tabular}{p{6.5cm}|c|c} 
\hline
DUCH Configuration & $I \to T$ & $T \to I$  \\ 
\hline\hline
Original & 0.836 & 0.824 \\ \hline
%\hline\hline
No adversarial loss  & 0.831 & 0.822 \\
%\hline
No quantization loss   & 0.818 & 0.800 \\
%\hline
No bit balance    & 0.828 & 0.826 \\ \hline
%\hline\hline
Contrastive loss: inter-modal    & 0.758 & 0.765 \\
%\hlineDUCH         & default parameters from \ref{sec:experiments-implementation} & 0.836 & 0.824 \\

Contrastive loss: inter-modal + image intra-modal    & 0.811 & 0.796 \\
%\hline
Contrastive loss: inter-modal + text intra-modal    &
0.813 & 0.815 \\
\hline
\end{tabular}
\end{table}
